Staged Animation Strategies for Online Dynamic Networks

Dynamic networks -- networks that change over time -- can be categorized into two types: offline dynamic networks, where all states of the network are known, and online dynamic networks, where only the past states of the network are known. Research on staging animated transitions in dynamic networks has focused more on offline data, where rendering strategies can take into account past and future states of the network. Rendering online dynamic networks is a more challenging problem since it requires a balance between timeliness for monitoring tasks -- so that the animations do not lag too far behind the events -- and clarity for comprehension tasks -- to minimize simultaneous changes that may be difficult to follow. To illustrate the challenges placed by these requirements, we explore three strategies to stage animations for online dynamic networks: time-based, event-based, and a new hybrid approach that we introduce by combining the advantages of the first two. We illustrate the advantages and disadvantages of each strategy in representing low- and high-throughput data and conduct a user study involving monitoring and comprehension of dynamic networks. We also conduct a follow-up, a think-aloud study combining monitoring and comprehension with experts in dynamic network visualization. Our findings show that animation staging strategies that emphasize comprehension do better for participant response times and accuracy. However, the notion of ``comprehension'' is not always clear when it comes to complex changes in highly dynamic networks, requiring some iteration in staging that the hybrid approach affords. Based on our results, we make recommendations for balancing event-based and time-based parameters for our hybrid approach.

==> Tex/scenario.tex <==
\section{Scenario: Computer Security Monitoring}
\label{sec:use_case}

Tools that allow users to examine data in real time or after the fact help the user identify behaviors and patterns of interest.
Once the behavior is characterized unambiguously, algorithms can be devised to automatically recognize it, but in mission-critical applications, it always helps to have a visual display of data so that new or unexpected patterns have a chance of being recognized.
% To create an algorithm that captures a behavior, it is required that the behavior is understood. 
% To understand a behavior, it requires for us to first be able to observe it.
% This is why tools that allow individuals to examine data either in real time or post event are important.
For example, CCTV footage is most often used to examine footage details after an event occurs, usually initiated by a live observation of something of interest (i.e. robbery, altercation).
On the other hand, security personnel also monitor CCTV footage in real time, looking for indicators of threatening events.
These ``indicators'' cannot be coded to be recognized by an automated system; it depends on the experience and perceptiveness of the security personnel monitoring the footage.
What determines \emph{when} the data needs to be observed is the importance of immediacy.
If an event of interest requires an immediate response from the viewer, and if the viewer has an understanding of the kind of behavior to anticipate, they can proactively observe the data.
% If the viewer knows beforehand that an event of interest will occur or require immediate response, such as a software launch, they can proactively observe the data.

A good example % of this interplay 
is computer security monitoring, as seen in the four cyber security data sources\footnote{\url{https://csr.lanl.gov/data/cyber1/}} within the Los Alamos National Laboratory's (LANL) corporate, internal computer network.
One data category of interest concerns network flow events.
These events indicate network connections between computers and contain relevant information such as time of connection, duration of connection, amount of information moved, and the protocol used.
% One of these types of data sources is a network flow event, which tracks network connection between computers and contains information such as time, duration, amount of information moved, and the protocol.

The authors of the network flow event dataset point out that ``compromise events'' are often intentionally created by authorized attackers to test network security~\cite{akent-2015}.
In their dataset of events spanning 58 days, 749 such compromise events occur, and are recorded with information such as \emph{domain}, \emph{source computer}, and \emph{destination computer}.
They observe that models are yet to be created to automatically identify some of the compromise events that are recorded in this dataset.
Currently, there exist some forms of attacks and malicious behavior in this dataset, the indicators of which have not yet been successfully validated or correlated.
This further underscores the need for compromising events to first be observed and understood.
Depending on the sensitivity of the data, this type of dataset might need live monitoring with in addition to other means of tracking such events.

% During the 58 days, a number of compromise events exist. These events were intentionally created to test the security of the computers and user accounts within the enterprise network by a group of authorised attackers, commonly known as a red team. Based on the documented activity of the red team, 749 authentication events are known to have been performed by the red team using stolen user credentials. These events include time, user with domain, source computer and destination computer are included. Other indicators of compromise may exist throughout the β data set, but have not been validated or correlated.We believe this initial, yet incomplete, compromise labelling will provide significant opportunity for a variety of research outcomes. However, while there is important value in developing models for “finding the bad guy” in the data set, we hope that the research community will use the β data set for broader research endeavours as well.

% As the authors of the data set pointed out, they have compromising events that occur within these data sets that are intentionally created, commonly known as red team~\cite{akent-2015}.
% They also point out that other compromising points may exist within this data set, but they have 
% This stresses the importance of e


% * First discuss the importance of streaming in context of dynamic

% * Follow up by stating there is similarity between these that we can look for it for examples of data sets. \
% * go through this similarities 
% * Finish off with LNALL data set and our use in the user study.




%we chose to use 5, but if another number is chosen, it would just shift the heat map staircase down and left.

% Tarik to write about how a computer network coming under attack can be
% visualized, and how a dynamic network visualization will help.

%Points to discuss
% To create an algorithm to capture a behavior first requires it to be understand. And to be understand requires it to be observed. 
% Algorithms will not capture every behavior. Still requires humans to note points of interest. What makes someone observer or choose to reply of section of the data. Either a algorithm or person points of that it is interesting. 
%Its not about having 100% accuracy, human will miss some kind of behavior. But an algorithm is only going to be as good as the individual who designed it.  
% CTT camera are used for more postmortem  
% To take a note that data is interesting in the first case requires the exploration(viewing it once) to determine the outcome
% Importance of immediacy: Being able to recognize a pattern quickly to be able to act.  
    % Conversations between a group or individual might be necessary to view in real time. So actions can be taken in timely manner.
    % Topic trending: Paying attention to development of topics over time.
    
% The translation from offline and online is not one to one but it quite similar. Data applicable to offline can also me applicable to offline.
% Specific types of dynamic social networks that have been investigated are, for example, textual online conversations such as chats [PT10], online communities [ATMS*11], the activity and interest of bloggers [IYTK12], the development of character relationships in literature [IA12, OKK13] or the propagation of microblogging messages [LQC*13]. Studying the evolution of these networks might support answering sociological and psychological questions, could help historians and literature scholar.

% Already in 1995, Kimelman et al. [KLRZ95] discuss the problem of visual complexity for visualizing program executions. Also visualizing the execution dynamics of software, others depict the information flow between processes [ET03], object interactions [GLW06], dynamic call graphs [BMR*12, BBV*12] or objects migrating between hosts [FT08a]. In addition to execution, another dynamic aspect of software that can be visualized is its evolution—the changes applied to software systems over time:

% When running systems and making sure everything functions. Requires real-time observation to determine if it should be stopped. Release of new software, and watching the traffic caused.(So points in time where its important to observe the launch of something(like software or run).

% * I need to discuss the LNALL dataset.

%* Structure



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

